Continuous-Time Gaussian Process Motion-Compensation for Event-vision Pattern Tracking with Distance Fields

This work addresses the issue of motion compensation and pattern tracking in event camera data. An event camera generates asynchronous streams of events triggered independently by each of the pixels upon changes in the observed intensity. Providing great advantages in low-light and rapid-motion scenarios, such unconventional data present significant research challenges as traditional vision algorithms are not directly applicable to this sensing modality. The proposed method decomposes the tracking problem into a local SE(2) motion-compensation step followed by a homography registration of small motion-compensated event batches. The first component relies on Gaussian Process (GP) theory to model the continuous occupancy field of the events in the image plane and embed the camera trajectory in the covariance kernel function. In doing so, estimating the trajectory is done similarly to GP hyperparameter learning by maximising the log marginal likelihood of the data. The continuous occupancy fields are turned into distance fields and used as templates for homography-based registration. By benchmarking the proposed method against other state-of-the-art techniques, we show that our open-source implementation performs high-accuracy motion compensation and produces high-quality tracks in real-world scenarios.

==> reviews.tex <==
Notable comments

### REVIEWER 1

The method is also relatively complex, with a lot of
different stages and optimizations. While the text does
encompass this, it would be helpful for the reader to
include a diagram or algorithm to summarize this. Fig. 2
does this to some extent, but I feel this summarizes at too 
high of a level, and does not explain the method properly.

The authors also do not discuss the run-time of this
method, which seems critical for event cameras where low 
latency is one of the major selling points. 



### REVIEWER 2

There are however a couple of issues that potentially weigh
down the above contribution:
- It seems the CT GP motion compensation method was 
evaluated only synthetic data (Section IV.A). This could
have been motivated by the need to obtain accurate ground
truth, but I think the text should provide justifications.
- While building on top of the CT GP motion compensation
method to yield a 2D tracking algorithm is useful, I feel
adding the other components (homography registration and 
pattern tracking) somewhat dilutes the main contributio
(those two additional components seemed independent to the 
motion compensation method anyway). I feel it would have
been better if more attention is devoted to CT GP motion
compensation (e.g., more examples, details on the 
algorithm, experiments on real data).


### REVIEWER 3


The presentation of the algorithms could be made more
accessible to readers without expert knowledge in Gaussian
Processes. It is hard to conceptualise how the model and
hyperparameters extract the velocities from the events. An
additional figure may help. I suggest, a full study on the
comparison of this method v.s. full image-based motion
compensation by contrast maximisation could be sufficient
for a stand-alone publication.


How does the Gaussian Process compare to other models for
velocity estimation - e.g. is it better than regression of
a plane to fit the spatio-temporal patterns? Is the
distribution of the events really Gaussian? Similarly, how
do distance fields compare to something like ICP for
pattern registration?

Results are not very conclusive as to the benefit of your
algorithm over prior SOTA. The simulated data may not
express correct noise characteristics at the spatial scale
that the algorithm is operating. The real camera data only
shown 2 seconds of 3 different datasets. The video isn't
clear why the author's algorithm is better than the others.


To further demonstrate feature tracking algorithms with
event cameras, results may need to mature showing real
practical benefits in robotics applications.

It isn't really clear how the components were used in the
ablation study? I guess Ours-SE(2) used only the motion
parameters of the motion compensation as the estimate of
motion? The Ours-B2B didn't perform motion compensation,
but estimated homographies for uncompensated events? Please
clarify.

Fig. 5. I didn't understand the metric "ratio of inlier
tracks" - i.e. what are the variables used in the ratio?
Please show more results clearly showing why your algorithm
outperforms others?

The choice of batch-sizes seems arbitrary and I am
concerned the parameters must be tuned for each dataset.
How sensitive is the algorithm to the choice of batch-size
(for different datasets and environments). Can you
guarantee real-time operation with these batches, otherwise
what kind of "offline" applications do you suppose that the
algorithm would be useful for. The algorithm seems quite
heavy limiting its use for real event streams for moving
cameras - the computational improvements will strengthen
the paper.

Check the references - some names are missing and some
arXiv papers have been published.


### REVIEWER 4

1. One potential limitation (which may apply to most
motion-compensation based algorithms) is that the method
will likely perform poorly in the absence of strong edges.
It is not entirely clear to me if the distance filed or the 
skeletonization approach as shown on Fig.3 will allow for 
accurate tracking in low contrast settings. Another
possible failure mode would possibly be the noise? I would
suggest performing an extensive analysis of the algorithm
performance in such scenarios.

2. On the video, the number of tracks seem to be extremely
small, even for rival methods. Was there a parameter
tuning? How were the experiments set up exactly? I think a
separate section with descriptions and implementation
details, or links to the code would help here.

3. Some discussion on why an SE(2) model was chosen would
be useful; e.g. in [https://protect-au.mimecast.com/s/hMaMCjZ1nVUEkQ8gFYnSyS?domain=arxiv.org]
authors use a 5-parameter model on a more complicated
scene. How does your approach compare to that paper? Some
discussion / comparison would be useful as SE(2) might seem
as a big limitation of the presented method.

3. Overall, the evaluation could be improved with a bigger
selection of scenarios and datasets. The planar scenes
chosen are quite primitive and more datasets are publically
available that have trackable patterns. How will your methd
perform on motion segmentation tasks? E.g. EVIMO
(https://protect-au.mimecast.com/s/AyovCk81oVHlZz9gCyjNP4?domain=better-flow.github.io) has 
plently of interesting scenarios, including high-noise
ones. As mentioned above, tolerance to noise is a valuable
metric for event-based camera algorithms.
